Almost Surely $\sqrt{T}$ Regret for Adaptive LQR

The Linear-Quadratic Regulation (LQR) problem with unknown system parameters has been widely studied, but it has remained unclear whether $\tilde{ \mathcal{O}}(\sqrt{T})$ regret, which is the best known dependence on time, can be achieved almost surely. In this paper, we propose an adaptive LQR controller with almost surely $\tilde{ \mathcal{O}}(\sqrt{T})$ regret upper bound. The controller features a circuit-breaking mechanism, which circumvents potential safety breach and guarantees the convergence of the system parameter estimate, but is shown to be triggered only finitely often and hence has negligible effect on the asymptotic performance of the controller. The proposed controller is also validated via simulation on Tennessee Eastman Process~(TEP), a commonly used industrial process example.

==> Makefile <==
.PHONY: all clean force

all: main.pdf response.pdf response2.pdf response3.pdf counterexample_standalone.pdf

main_arxiv.pdf: force
	sed -i 's/\\setboolean{tacVersion}{true}/\\setboolean{tacVersion}{false}/' main.tex
	if [ -f main.pdf ]; then mv main.pdf main_backup.pdf; fi
	latexmk -shell-escape -synctex=1 -interaction=nonstopmode -file-line-error -pdf main.tex
	mv main.pdf main_arxiv.pdf
	if [ -f main_backup.pdf ]; then mv main_backup.pdf main.pdf; fi


main.pdf: force
	sed -i 's/\\setboolean{tacVersion}{false}/\\setboolean{tacVersion}{true}/' main.tex
	latexmk -shell-escape -synctex=1 -interaction=nonstopmode -file-line-error -pdf main.tex
	sed -i 's/\\setboolean{tacVersion}{true}/\\setboolean{tacVersion}{false}/' main.tex

main.aux: main.pdf
	sed -i -E 's/(\\newlabel\{[^}]+\}\{\{[^}]+\}\{[^}]+\}).*/\1{{}}{}}/g' main.aux

counterexample_standalone.pdf: main.aux force
	latexmk -shell-escape -synctex=1 -interaction=nonstopmode -file-line-error -pdf counterexample_standalone.tex

response.pdf: main.aux force
	latexmk -shell-escape -synctex=1 -interaction=nonstopmode -file-line-error -pdf response.tex

response2.pdf: main.aux force
	latexmk -shell-escape -synctex=1 -interaction=nonstopmode -file-line-error -pdf response2.tex

response3.pdf: main.aux force
	latexmk -shell-escape -synctex=1 -interaction=nonstopmode -file-line-error -pdf response3.tex

clean:
	latexmk -C
	rm -f tikzcache/figures/*.tex.*

